Improved Revenue Bounds for Posted-Price and Second-Price Mechanisms

We study revenue maximization through sequential posted-price (SPP) mechanisms in single-dimensional settings with $n$ buyers and independent but not necessarily identical value distributions. We construct the SPP mechanisms by considering the best of two simple pricing rules: one that imitates the revenue optimal mchanism, namely the Myersonian mechanism, via the taxation principle and the other that posts a uniform price. Our pricing rules are rather generalizable and yield the first improvement over long-established approximation factors in several settings. We design factor-revealing mathematical programs that crisply capture the approximation factor of our SPP mechanism. In the single-unit setting, our SPP mechanism yields a better approximation factor than the state of the art prior to our work (Azar, Chiplunkar & Kaplan, 2018). In the multi-unit setting, our SPP mechanism yields the first improved approximation factor over the state of the art after over nine years (Yan, 2011 and Chakraborty et al., 2010). Our results on SPP mechanisms immediately imply improved performance guarantees for the equivalent free-order prophet inequality problem. In the position auction setting, our SPP mechanism yields the first higher-than $1-1/e$ approximation factor. In eager second-price (ESP) auctions, our two simple pricing rules lead to the first improved approximation factor that is strictly greater than what is obtained by the SPP mechanism in the single-unit setting.

==> related1.tex <==
\section{Related Work}
\label{sec:related}
\paragraph{Prophet Inequalities} The work on posted price mechanisms has been 
intimately connected to the work on prophet inequalities. In the classic 
prophet inequality setting, $n$ independent (but not necessarily identical) 
random 
variables arrive in an adversarial sequence, and after each random variable 
arrives, the gambler faces two choices: accept the random variable and stop, or 
reject 
and continue. The objective is to maximize the expected value of the random 
variable selected by the gambler. Performance is measured by the ratio of the 
gambler's choice to the expected value of the maximum of $n$ random variables 
(the 
objective that a prophet with complete foresight can obtain). Other important 
variants of this standard 
setting are the ones where the random variables arrive in a uniformly random 
order (known as the \emph{prophet secretary} or the \emph{random ordered 
prophets} problem), and the one where the 
random variables can be picked by the player in her desired order (known as 
\emph{ordered prophets}).

\paragraph{Adversarial and i.i.d. prophets.} The study of prophet inequalities 
began in the 1970's by Krengel and 
Sucheston~\cite{KS77,KS78,Kennedy87}.~\citet{HK81} show that in the 
adversarial setting, the gambler can obtain at least $\frac{1}{2}$ of the 
expected value obtained by a prophet. This constant cannot be 
improved, even if the prophet were allowed to use adaptive strategies, and even 
if we make large market assumptions like each distribution occurring at least 
$m$ times for any arbitrarily large $m$~\cite{AEEHKL17}. 
Later~\cite{samuel-cahn1984} showed that the same $2$-approximation 
can be obtained by a simple threshold policy, that posts a single threshold and 
accepts the first random variable to exceed the threshold. This 
$\frac{1}{2}$-approximation was later used by~\citet{chawla2010multi} to give a 
$\frac{1}{2}$-approximation for the posted-prices mechanism when the buyers 
arrive in an adversarial order. When the random 
variables are i.i.d,~\citet{HK82} showed that the gambler can obtain at least 
$1-\frac{1}{e}$ of the prophet's value, and also show examples that prove that 
one cannot obtain a factor beyond $\frac{1}{1.342}\sim 0.745$.~\citet{Kertz88} 
later conjectured that $\frac{1}{1.342}\sim 0.745$ is the best possible 
approximation. The first formal proof that one can go beyond $1-\frac{1}{e}$ 
was given by~\citet{AEEHKL17} who give a $0.738$ for all $n$ beyond a certain 
constant $n_0$. Simultaneously and independently,~\cite{correa2017posted} 
showed a 
$0.745$ 
approximation for this problem, there by completely closing the gap. 

\paragraph{Ordered prophets.}~\citet{chawla2010multi} give a $1-\frac{1}{e}$ 
approximation for the SPM problem, and while it was unknown at that time 
recently~\cite{correa2017back} showed that any approximation for SPMs implies 
the same 
approximation for ordered prophets as well. This bound of $1-\frac{1}{e}$ was 
recently surpassed by~\cite{azar2017prophet} to $1-\frac{1}{e} + 0.0025$, and 
their bound extends to random order prophets as well. The bound of 
$1-\frac{1}{e} + 0.022$ that we give in this paper for SPMs, which implies 
the same bound for ordered prophets by the result of~\citet{correa2017back}, is 
the best 
known bound for ordered prophets so far.

\paragraph{Random order prophets / prophet secretary.} The random order prophet 
inequality problem, 
or the prophet secretary problem was first studied 
by~\citet{esfandiari2017prophet}, where they 
show a $1-\frac{1}{e}$ approximation for large $n$. They also show that with a 
single threshold it is impossible to get better than a 
$\frac{1}{2}$-approximation.~\citet{correa2017posted} show that one can obtain 
a $1-\frac{1}{e}$ approximation for every $n$ with non-adaptive thresholds. 
Finally~\cite{azar2017prophet} show that one can obtain a $1-\frac{1}{e} + 
0.0025$ approximation for any $n$. 

\paragraph{Prophets with large $n$.} When $n$ is very large, and when each 
distribution occurs at least a constant $m_0$ times, ~\citet{AEEHKL17} show 
that one 
can obtain a $0.738$ approximation for ordered prophets, and the same 
approximation for prophet secretary when we have at least $c_0\log(n)$ copies 
of each distribution.

\paragraph{Posted prices, prophet inequalities and generalizations.} The 
connection between prophet inequalities and mechanism design was initiated 
by~\citet{HKS07}, where they interpreted the prophet inequality algorithms as 
being truthful mechanisms for online auctions.~\citet{CHK07} give a 
$4$-approximation to the single agent $n$ items unit-demand pricing problem, 
via upper bounding the revenue of the multi-parameter setting by that of the 
single item $n$ buyers single-parameter 
problem.~\citet{chawla2010multi,chawla2010randomized} 
further this connection, and develop constant fraction approximations for 
several multi-parameter unit-demand settings, by developing constant factor 
approximations to the corresponding single-parameter posted price settings 
through connections to prophet inequalities.~\citet{yan2011mechanism} makes a 
connection between the revenue of SPM and correlation gap for submodular 
functions~\cite{agrawal2012price}.~\citet{TEGMM10} develop a PTAS for 
computing the optimal adaptive and non-adaptive SPMs in a $k$-item single 
parameter setting.~\citet{KW12} generalize the prophet inequalities result to 
the matroidal environment, and use this to give improved approximations for the 
multi-parameter unit-demand mechanism design problem. For other generalizations 
of posted-prices and prophet inequalities to combinatorial settings, 
see~\cite{polymatroidprophets,FGL15,RS17,EHKS18,prophetsmadeeasy}.

\paragraph{Second price auction with personalized reserve prices.}~\citet{HR09} 
study the question of approximating the optimal mechanism's revenue via Vickrey 
auction with personalized reserve prices, and show that for regular 
distributions, the second price auction with the so-called monopoly reserve 
prices yield a $2$-approximation for regular distributions, and that for 
irregular distributions no constant factor approximation is possible with the 
monopoly reserves.~\citet{paes2016field} study the question of computing the 
optimal personalized reserve prices in a correlated distribution setting, and 
show that the problem is NP-hard. The hardness status of this problem is 
unknown for independent distributions.~\citet{RW16} show that this problem is 
APX-hard for correlated distributions and give a $\frac{1}{2}$-approximation. 
Second price auctions with lazy personalized reserve prices are incomparable to 
second price auctions with eager reserve prices for general correlated 
distributions, but are within a factor $2$ of each other~\cite{paes2016field}. 
However, when the distributions are independent, or when the 
bidders are symmetric,~\citet{paes2016field} show that the optimal eager 
auction dominates the revenue of the optimal lazy auction.
